Edit-Run Behavior in Programming and Debugging

As developers program and debug, they continuously edit and run their code, a behavior known as edit-run cycles. While techniques such as live programming are intended to support this behavior, little is known about the characteristics of edit-run cycles themselves. To bridge this gap, we analyzed 28 hours of programming and debugging work from 11 professional developers which encompassed over three thousand development activities. We mapped activities to edit or run steps, constructing 581 debugging and 207 programming edit-run cycles. We found that edit-run cycles are frequent. Developers edit and run the program, on average, 7 times before fixing a defect and twice before introducing a defect. Developers waited longer before again running the program when programming than debugging, with a mean cycle length of 3 minutes for programming and 1 minute for debugging. Most cycles involved an edit to a single file after which a developer ran the program to observe the impact on the final output. Edit-run cycles which included activities beyond edit and run, such as navigating between files, consulting resources, or interacting with other IDE features, were much longer, with a mean length of 5 minutes, rather than 1.5 minutes. We conclude with a discussion of design recommendations for tools to enable more fluidity in edit-run cycles.

==> sections/oldResult.tex <==
\section{results}
In this section we report challenges developers faced while using debugging strategies. These challenges are enumerated with examples to illustrate how developers struggled and attempted to overcome these challenges. 
\subsection{Formulating and Testing Hypotheses}
Developers use clues (e.g., source code, programming output) and expertise to hypothesize what might cause the defect to occur. They then seek to test these hypotheses to confirm or reject them. We identified four challenges developers face in formulating and testing hypotheses. 



%https://youtu.be/gW9s44bzEIU?list=PLk8nR1R4Kasg1cs7poJ0uiSsUzSIdoUX3&t=4004
%https://youtu.be/ijI4Rcus1Cs?t=5540
%https://youtu.be/L2DJhwANoUQ?t=4698
\subsubsection{Formulating hypotheses with lack of clear clues}

When a defect produces poor feedback(i.e., confusing error messages and behavior) and the developers could not relate the defect's behavior to similar familiar defects based on their experience, developers struggled to formulate a correct hypothesis. 

\textbf{Examples:} D1 faced a defect that made his search functionality showed a ``no result found'' message no matter the input was. He had multiple hypotheses that he tested and found that they were incorrect. He decided to put several log statements to seek any information about why the search functionality was not finding any result. Unfortunately, the log information provided little to no insight about the defect as most of them did not execute in the first place. While he was searching in StackOverflow and debugging the code,  he suddenly said ``actually could it be'' and switch the terminal to find out that there was an old server running his old code. ``OK, I spent the last ten minutes debugging this problem and it turns out that I had an older version of the code running on the same port, crap''. ``This is much better'' after killing the old server, and the output now showed an error message.

%https://youtu.be/9vrhpgeRlqA?list=PLpXAyWkDQy43xYWkRVDvxyPxhLeHDxdmg&t=5877

%D2 was working on making his face recognition application run in mutithreading environment. After successfully compiling his code and running it, the face recognition suffered from sever performance issues. The only feedback he got from the program was ``Converter dropped frame!''. His initial hypothesis that his implementation of queue frame is incorrect. He went to the example he copied from StackOverflow and checked that everything was correctly implemented. He then tried to launch the profile to check why his code is slow. Unfortunately, the profile crashed multiple times and did not work. After nof finding any information about why his code was slow, he decided to stop working and finished the stream and return back to it later in the future.

%https://youtu.be/9vrhpgeRlqA?list=PLpXAyWkDQy43xYWkRVDvxyPxhLeHDxdmg&t=5851
%https://youtu.be/9vrhpgeRlqA?list=PLpXAyWkDQy43xYWkRVDvxyPxhLeHDxdmg&t=8180
D10 had similar experience in which he was debugging a defect that caused a performance issue for cURL reported by another developer through GitHub issues. However, since the defect was not crashing the library, there was no error message to help him to hypothesize. What puzzled him more was that changing part of the code that he thought should not have any impact on the performance was impacting the performance. ``I am totally perplexed ... it is hard to figure out. Why would it matter if I sent a smaller [HTTP] POST?''. He spent nearly an additional hour of debugging before he had a hypothesis and started to write code to test it. 

%https://youtu.be/mMGWUPBGFoM?t=2468
%https://youtu.be/gW9s44bzEIU?list=PLk8nR1R4Kasg1cs7poJ0uiSsUzSIdoUX3&t=3120
There were two other developers (D4 and D7) who struggled with forming hypotheses because of lack of clues, but what was different in their situations was that instead of seeking information about the defect through switching debugging strategies, they got hypotheses suggestions from other developers who were watching them while debugging. This not only made them active testing hypotheses instead of getting puzzled by why such defect happened, but also helped in finding the defect and fixing it. D4 Was debugging a defect that produced a ``horrible'' error message that made his game crashed immediately. The developer got confused until another developer who was watching pointed out that he might not have copied the image to the correct file distention, which was the correct hypothesis. In case of D7, the hypotheses suggested by another developer did not help in fixing the defect but to understand that the defect was due to a limitation of a third party library, which made her abandoned the library in favor of rewriting the necessary logic herself.  

\begin{figure}
\centering
  \includegraphics[width=\linewidth, keepaspectratio, clip]{sections/figures/Example2.jpg}
  \captionof {figure}{ The developer has set the browser output on the left and his code editor on the right. His setting made his cod edit reflect on the output instantly, enabling him to test hypotheses faster.}
  \label{fig:example2}
\end{figure}
\subsubsection{Testing and refining general hypotheses}
Defects may produce error messages or behavior that do not directly suggest the cause of the defect but enable developers to form general hypotheses about what might cause the defect to occur. The challenge, in this case, is developers need to continually test and refine their general hypothesis until they find the actual cause of the defect, which may slow down the process due to the need to compile, run and reproduce the defect each time.
%https://youtu.be/T_6q12hoHug?list=WL&t=9563
\textbf{Examples:} D5 was working in building a responsive website. His development environment setup made the result of his code editing showed in the browser instantly after each time he saved the changes. While working, he noticed that the iframe elements in the website were not responsive to different screen sizes as the other HTML elements. He seemed to know that the cause of the defect was due to missing CSS properties but did not know what the properties were. Thus, he brought up the browser side by side to his code editor and started editing CSS code and watching the effect of his edit in the browser. This enables him to test and refine hypotheses faster and eventually fix the defect (Figure \ref{fig:example2}).



%https://youtu.be/s9cHvUQM5vU?t=813
On the other hand, D8 was debugging a defect with a general hypothesis that the problem is inside one function that comprised multiple of asynchronous calls. He was not sure which one of these calls caused the problem. So he spent nearly 20 minutes adding logs statements, removing a line of code and experimenting with different parameters, requiring him to compile, rerun the program, and manually interact with the application to test the result of each new edits. This made refining and testing his hypotheses very slow and expensive. The developer gave up as he was not able to find the specific cause of the defect and moved to debug another issue. 


%https://youtu.be/L2DJhwANoUQ?t=2339
\subsubsection{Testing hypotheses about the correctness of the output}
Developers may not be able to tell if the output of a program is the correct output or not. Thus, they may hypothesize that the output is correct and seek to test this hypothesis. Unlike hypotheses about the cause of a defect which can be tested with editing the code or observing its state, We found that developers test hypotheses about the correctness of the output by running another similar but correct applications and compare the output of these applications with their program's outputs. The process of finding another program that produces the correct result was sometimes challenging.    


\textbf{Examples:} D8 was debugging a defect that made the value of one variable to 400. This value was a result of a bit shifting operation that the developer hypothesized to be correct. To test his hypothesis, he opened a well-known command line calculator (bc) and checked if the result of the same bit shifting operation in this calculator equaled to 400.

D1 experience was more difficult than D8. He code was fetching data from Reddit website and  saving hundreds of posts successfully. However, he was not sure that the posts he downloaded were legitimate and complete. He hypothesized that his code was working as expected, but he wanted to double check. He went to the Reddit website and needed to figure out how to construct the same query he did programmatically through the web interface. He then started comparing some of the posts he downloaded with the posts displayed with the search result from the website.

%https://youtu.be/AWLzSIFbbeA?list=PL18yrUuMk-zmFPlagLPyC2TNqjJixvxJR&t=218
%https://youtu.be/xxmNU-Myokc?t=2797
\subsubsection{Testing hypotheses in complicated settings}
Modern software is built in an environment that depends on third-party libraries and tools. When confronting a defect in such complicated settings, developers may hypothesize that the defect is due to these libraries or misuse of them and not in their core program logic. The challenge of testing such hypotheses is that it may require developers to separate the impact of the rest of their code from the output of these libraries and tools. This is closely related to how Delta debugging works \cite{orsowoda2006, Cleve2005LocatingCO, Zeller2002}, but instead of simplifying the program by removing code or input based on test cases, we found that developers test these hypotheses by constructing a simple program from scratch to only test these hypotheses.

\textbf{Examples:} While D1 was testing his implementation that attempted to use third-party library to persist objects in files, his code crashed with an error message. After reading the error message, the developer hypothesized that the defect might be related to misuse of the library's API and not on another part of the code. To test his hypothesis, he created a simplified program that stored and read an object using the library, checking if his use of the library was correct. He was able to reject his hypothesis and confirm that his use of the library was correct, suggesting the defect was elsewhere.

D2 had a similar situation in which he was trying to compile C++ code but got an error message. He wanted first to validate the hypothesis that the compiler is configured correctly and would be able to compile any code. To do so, he created simple C++ code that print ``Hello World'' and tried to compile it. The code compiled correctly,  confirming his hypothesis that the problem was not with the compiler configuration.

\begin{figure}
\centering
  \includegraphics[width=\linewidth, keepaspectratio, clip]{sections/figures/Example1.jpg}
  \captionof {figure}{The source code for the server was not available for the developer to reason about its implementation. Instead, he called the server with several payloads with different sizes. He then started to reason about its behavior based on the output.}
  \label{fig:example1}
\end{figure}


\subsection{Reasoning about Code}
Developers may need to check their program state or understand its behavior while debugging. We found that reasoning about abstraction, the cost of doing dynamic reasoning, and hard to inspect and observe defects created challenges for developers while using debugging strategies that involve reasoning about code.

%https://youtu.be/9vrhpgeRlqA?list=PLpXAyWkDQy43xYWkRVDvxyPxhLeHDxdmg&t=4997
%https://youtu.be/8UzLuMiGs9s?t=3654
\subsubsection{Reasoning about abstraction} %D10 and D6
While reason about their program execution and state, developers may also want to understand how third-party APIs that they used in their program beehives internally. What usually happens, in this case, is that developers consult the APIs' official documentation to understand how the APIs behave and whether the defect is related to its behavior. We found that developers face a challenge when there is no official documentation or the documenting lacks the necessary details. In this case, developers either dive into the APIs' internal code to understand it or reason about its behavior by interacting with it if the code is not available to them.  

\textbf{Examples:} D10 was trying to understand how the server was behaving with differently sized payloads in order to understand a defect that caused cURL to suffer from a performance issue while fetching data from that server. As he had no access to the source code of the server, he tried to understand the behavior of the service by inspecting the request to and the response from that server. He made several different requests and used a visual tool to help him in understanding the data he collected (Figure \ref{fig:example1}). He was able then to conclude that the server might be the responsible for causing the defect.

D6 was trying to answer a question he had about API usage that might be related to the cause of a defect he was debugging. The API documentation did not have enough information to answer his question. However, unlike D10 who did not have access to the source code of the server, D6 had access to the library source code which helped him in answering his question about the API.
%https://youtu.be/8D97omdDEwA?list=WL&t=5843
%\begin{figure}
%\centering
%  \includegraphics[width=\linewidth, keepaspectratio, clip]{sections/figures/codeExample.pdf}
%  \captionof {figure}{}
%  \label{fig:example1}
%\end{figure}

\subsubsection{The cost of dynamic reasoning} %D2 and D3 D9
To understand the incorrect state and behavior of a program, developers may need to run and inspect the program (i.e., through debugger breakpoints or by inserting print statements) in forwards or backwards reasoning strategies. Defects in complex program may not manifest until the program have been running for a long time, requiring developers to step over long execution chain until exposing the incorrect state. While inspecting, developers may also need to rerun the program if they have decided to change part of the code or re-execute piece of the logic again. These made dynamic reasoning in some cases expensive. We found that some developers utilized existing debugging tools and techniques to avoid stepping through long execution and rerunning the program again when they decided to edit it.  

%https://youtu.be/sk6-sSjx7Bc?t=1915
%https://youtu.be/ijI4Rcus1Cs?t=5167
\textbf{Examples:} D3 was debugging a defect that crashed the program after it has been running for a while with an error message saying that variable \textit{X} had an invalid none-numeric value. Instead of using forewords reasoning and take all steps in the execution until the \textit{X} variable got a non-numeric value, D3 decide to do backward-reasoning starting from the point when \textit{X} got the non-numeric value. D3 did not know where the best starting point for doing backword-reasoning since \textit{X} was a global variable that was mutated in different locations. He decided to implemented a \textit{setter} method for \textit{X} that forced any mutation to its value to be done using this method. He then set an assertion inside that method that failed when the assigned value to \textit{X} was non-numeric. He configured the debugging tool to set a breakpoint when the assertion failed. He reran the program and waited until the assertion failed and the program halted on that exception. He went backwoods in the execution and were able to identify the defected calculation that caused  \textit{X} to get invalid value.

D9 was debugging a defect that caused Firefox browser to fail to load CSS sheets. He put a debugger statement after the code that was responsible for loading the CSS sheets and brought the Firefox DevTools and used the integrated REPL to check the values of several variables. What was interesting in his case that he wanted to change a specific piece of code and check its impact on the program state. Instead of editing the program and rerun it, he copied and edited the desired piece of code and then execute it in the REPL against the current state of the program. 

%https://youtu.be/9vrhpgeRlqA?list=PLpXAyWkDQy43xYWkRVDvxyPxhLeHDxdmg&t=2308
%https://youtu.be/sk6-sSjx7Bc?t=3381
%https://youtu.be/ijI4Rcus1Cs?t=5379
\subsubsection{Hard to inspect and observe defects} %D9, D10
Sometimes defects produce subtle incorrect behavior that is hard to observe or the inspection process is complicated due defected debugging tools. We found that developers alter the program behavior to make the inspection and observing these defects easier. 

\textbf{Examples:} D10 was debugging a defect that was hard to observe while the program only processes two URLs. He went and made the program process 10 URLs instead. ``With 10 URLs the defect is more noticeable because then it will spend one second per URL''. This made the program execute for a longer time, which helped the developer to understand the defect behavior quickly.

D9 had a situation in which the debugger was not halting the execution of the program completely, causing the web page he was inspecting to reload. To make sure that the program stop execution thoroughly, he went and inserted a sleep command that causes the main thread to pause for 41 hours after the debugger line. ``I hope this is going to give me enough time'' he commented.


\subsection{Seeking help}
When developers encounter an error message that they cannot understand or a fix to a defect that they do not know how to implement, they may seek help by browsing documentation on developer Q\&A websites such as StackOverflow. We found that developers faced challenges integrating suggested solutions into their existing code.  

%how to copy code and incorporate it to the code base D1 and D2 or not knowing what solution to if you face such error (incomplete help)
%https://youtu.be/8D97omdDEwA?list=WL&t=2793
\subsubsection{Integrating code snippet}
Developers used and share code snippets as suggested solutions to common defects. These code snippets can be found in Stackoverflow posts, the official documentation of an API, or technical articles. However, developers may face a challenge in how they incorporate these suggested fixes in their existing code as these code snippet usually presented in a simple example in which it lacks the full context about where it should correctly be placed. We found that developers used a try and error approach to figure out how to integrate these snippets with their existing codebase.

\textbf{Examples:} D2 got an error message that suggested the usage of micro in order to compile his code correctly. Mystified, he searched about how to use this micro on the internet. He found a code snippet from the official documentation that showed how to use that micro. However, he did not know exactly where to place the micro in his code.  His first attempt result in an error message: ``a template declaration cannot appear at black scope'' which suggested that he placed the code snippet in a wrong location in his codebase. ``Well, that super not helpful'' after reading the error message. After several trial and error and further research, he finally found how to integrate the micro in his code correctly.

%https://youtu.be/L2DJhwANoUQ?t=10179
D1 copied an error message and pasted into Google while he was debugging a defect related to the usage of a third-party library. He went to a StackOverflow post and found a code snippet that he thought might be the fix for the defect he was debugging. He copied the code snippet and pasted it in random place since he was not sure where the snippet should be placed in his code. The defect was not fixed as the same error message showed up again. He changed the location of the code snippet a couple of times but could not fix the defect. He decided to end the video stream at that point because he felt stuck.

%https://youtu.be/gW9s44bzEIU?list=PLk8nR1R4Kasg1cs7poJ0uiSsUzSIdoUX3&t=1934
%\subsubsection{information cluttering}
